1RXH J082623.6-505741: a new long-period cataclysmic variable with an evolved donor and a low mass transfer rate

We report the discovery of 1RXH J082623.6-505741, a 10.4 hr orbital period compact binary. Modeling extensive optical photometry and spectroscopy reveals a $\sim 0.4 M_{\odot}$ K-type secondary transferring mass through a low-state accretion disk to a non-magnetic $\sim 0.8 M_{\odot}$ white dwarf. The secondary is overluminous for its mass and dominates the optical spectra at all epochs, and must be evolved to fill its Roche Lobe at this orbital period. The X-ray luminosity $L_X \sim 1$-$2 \times 10^{32}$ erg s$^{-1}$ derived from both new XMM-Newton and archival observations, although high compared to most CVs, still only requires a modest accretion rate onto the white dwarf of $\dot{M} \sim 3 \times 10^{-11}$ to $3 \times 10^{-10} M_{\odot}$ yr$^{-1}$, lower than expected for a cataclysmic variable with an evolved secondary. No dwarf nova outbursts have yet been observed from the system, consistent with the low derived mass transfer rate. Several other cataclysmic variables with similar orbital periods also show unexpectedly low mass transfer rates, even though selection effects disfavor the discovery of binaries with these properties. This suggests the abundance and evolutionary state of long-period, low mass transfer rate cataclysmic variables is worthy of additional attention.

==> Makefile <==
# Manually set if this is an arXiv sumbission (needs .bbl file)
#ARXIV=no
ARXIV=yes

# Automated setup: try hard to find the main tex file and recognize its format: PDF figure, BibTeX...
TEXFILE_BASENAME = $(shell ls -S *.tex | head -n1 | sed 's:.tex::g')

PDFTEX := $(shell cat *.tex | cut -f1 -d"%" | grep 'includegr' | grep --quiet -e '.pdf' -e '.png' && echo 'yes' )
BIBTEX := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet 'bibliographystyle' && echo 'yes' )

MODIFY_BIBFILE_ULTRACOMPACT_REF := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'bibliographystyle.mnras_shortlisthack' -e 'bibliographystyle.supershort_numbers_oneline' && echo 'yes' )

MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING := $(shell cat *.tex | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'mnras' && echo 'yes' )

AAS_MANUSCRIPT_REQUIRING_US_SPELLING := $(shell cat *.tex | cut -f1 -d"%" | grep 'documentclass' | grep --quiet 'aastex' && echo 'yes' )

ANY_KNOWN_SOFTWARE_MENTIONED := $(shell cat *.tex | cut -f1 -d"%" | grep --quiet -e 'IRAF' -e 'MIDAS' -e 'AIPS' -e 'CASA' -e 'DS9' -e 'ds9' -e 'VaST' -e 'HEASoft' -e 'HEASOFT' -e 'HEAsoft' -e 'Fermitools' && echo 'yes' )

all: info clean check_utf8 check_spell check_no_whitespace check_coma_instead_of_period check_extra_white_space try_to_find_duplicate_words shorten_journal_names_bib check_british_spelling check_us_spelling check_software_small_capitals $(TEXFILE_BASENAME).pdf

info:
	echo "Starting the ultimate LaTeX Makefile"
	echo "TEXFILE_BASENAME= "$(TEXFILE_BASENAME)

clean: 
ifeq ($(ARXIV),yes)
	# do not remove .bbl file for arXiv submission
	rm -f $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~
else
	# remove .bbl file and everything else
	rm -f $(TEXFILE_BASENAME).bbl  $(TEXFILE_BASENAME).pdf $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi $(TEXFILE_BASENAME).log $(TEXFILE_BASENAME).aux $(TEXFILE_BASENAME).blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf $(TEXFILE_BASENAME).out $(TEXFILE_BASENAME).teximulated mn2e.bst_backup missfont.log *~
endif

check_utf8: $(TEXFILE_BASENAME).tex
	# Display any non-ASCII UTF8 characters higlighting them with color
	cat $(TEXFILE_BASENAME).tex | { grep --color=always '[^ -~]\+' && exit 1 || true; }
	# Check that the TeX file type is not Unicode
	file $(TEXFILE_BASENAME).tex | { grep Unicode && exit 1 || true; }

check_spell: $(TEXFILE_BASENAME).tex
	# Case-insensitive search
	cat $(TEXFILE_BASENAME).tex | sed 's:the A config::g' | sed 's:binary tree::g' | { grep --color=always --ignore-case -e 'compliment' -e 'complimented' -e 'ile up' -e 'ile~up' -e ' can will ' -e ' may can ' -e ' may will ' -e ' a the ' -e ' the a ' -e ' whited ' -e 'neutrons star' -e 'hotpot' -e ' rang ' -e 'has be seen' -e 'synchroton' -e 'hight' -e 'far from being settled' -e 'recourses' -e 'wile' -e 'will allows' -e ' tree ' -e ' an new' -e 'data is ' && exit 1 || true; }
	# Case-sensitive search
	cat $(TEXFILE_BASENAME).tex | sed 's:the A config::g' | { grep --color=always -e 'x-ray' -e ' tp ' && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'countrate' && echo "SHOULD BE count rate" && exit 1 || true; }
	# Use \b to match on "word boundaries", which will make your search match on whole words only.
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always '\bgenue\b' && echo "SHOULD BE genuine" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'maid' && echo "DID YOU MEAN made ?" && exit 1 || true; }

check_no_whitespace: $(TEXFILE_BASENAME).tex
	#  cut -f1 -d"%" -- ignore everything after %
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	#
	# period      sed 's:[A-Z].[A-Z].::g' will allow for two capital letter combinations like initials K.S.
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | sed 's:R.A.::g' | sed 's:L.A.Cosmic::g' | sed 's:\\.M::g' | sed 's:Obs.ID::g' | sed 's:U.S.::g' | sed 's:H.E.S.S.::g' | sed 's:J.D.L.::g' | sed 's:K.V.S.::g' | sed 's:E.A.::g' | sed 's:Ras.Pi::g' | sed 's:Ph.D.::g' | sed 's:P.O.::g' | sed 's:[A-Z].[A-Z].[A-Z].::g'  | sed 's:[A-Z].[A-Z].::g' | { grep --color=always -e '\.[A-Z]' && exit 1 || true; }
	# two periods
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\.\.' && exit 1 || true; }
	# coma periods
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\,\.' && exit 1 || true; }
	# some journal styles allow ".," combination: "e.g.,"
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\.\,' && exit 1 || true; }
	# two comas
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep --color=always -e '\,\,' && exit 1 || true; }
	#
	# White space between Fig. and ref
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Fig\.\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Fig\\ref' && echo "SHOULD BE Fig.~\\ref{}" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Figure\\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always 'Figure \\ref' && echo "SHOULD BE Figure~\\ref{}" && exit 1 || true; }
	# White space before \cite
	cat $(TEXFILE_BASENAME).tex | sed 's:\\protect\\citeauthoryear::g' | { grep --color=always '[a-z]\\cite' && echo "NO WHITE SPACE BEFORE \\cite" && exit 1 || true; }

check_extra_white_space: $(TEXFILE_BASENAME).tex
	cat $(TEXFILE_BASENAME).tex | { grep --color=always ' \.' && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | { grep --color=always ' \,' && exit 1 || true; }

check_coma_instead_of_period: $(TEXFILE_BASENAME).tex
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | grep -v -e 'Uni' -e 'Obs' -e 'Inst' -e 'The Netherlands' -e 'The United' | { grep --color=always -e '\,The' -e '\, The' && exit 1 || true; }

try_to_find_duplicate_words: $(TEXFILE_BASENAME).tex
	# Catch word repeats in one line
	# The old version that doesn't catch everything
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | grep -v -E '[0-9]cm' | grep -v -E '[0-9]in' | grep -v -e '&' -e 'textwidth' -e 'includegraphicx' -e 'includegraphics' -e 'tabular' | { egrep "(\b[a-zA-Z]+) \1\b"  && exit 1 || true; }
	# The new experimental version
	#  sed -e 's/\[[^][]*\]//g' -- ignore everything between []
	#  sed -e 's/{[^{}]*}//g'   -- ignore everything between {}
	# mess 'caption{}' and 'captionbox{}' as we still want to check for repeated words in captions
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ein --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	# Last-trench effort -- just grep for the most common repetition
	cat $(TEXFILE_BASENAME).tex | { grep --color=always ' the the ' && exit 1 || true; }
	#
	#
	# Checking for repeated words over linebreaks
	# We do not exclude comments, so line numbers will be correct
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	#  sed 's/%.*$//'    -- remove everything after %
	#  sed '/^[[:space:]]*$/d' -- remoove empty lines
	# The output line nubers may not be exact as we skip comment lines
	cat $(TEXFILE_BASENAME).tex | sed 's:\\it : :g' | sed 's:\\em : :g' | sed 's:\\bf : :g' | sed 's/%.*$$//' | sed '/^[[:space:]]*$$/d' | awk 'BEGIN{getline l;} {combined=l " " $$0; printf(" %.5d - %.5d: %s\n",FNR-1,FNR, combined); l=$$0;}' | grep -v 'tabular' | sed 's:caption{::g' | sed 's:captionbox{::g' | sed -e 's/{[^{}]*}//g' | sed -e 's/{[^{}]*}//g' | sed -e 's/\[[^][]*\]//g' | sed -e 's/\[[^][]*\]//g' | { grep -Ei --color  "\b(\w+)\b\s*\1\b" && exit 1 || true; }
	
# This hack will modify the .bib file replacing some long journal names if we are using mnras_shortlisthack.bst style
shorten_journal_names_bib:
ifeq ($(MODIFY_BIBFILE_ULTRACOMPACT_REF),yes)
	# Modify .bib
	echo "I WILL RUIN THE BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
	# If the bibfile looks unmodified, save a backup copy
	cat $(TEXFILE_BASENAME).bib | { grep -e '{ATel}' -e '{RNAAS}' -e '{AN}' || cp -v $(TEXFILE_BASENAME).bib $(TEXFILE_BASENAME).bib_backup_long_journal_names ; }
	# Do the actual modification
	cat $(TEXFILE_BASENAME).bib | sed 's:{The Astronomer.s Telegram}:{ATel}:g' | sed 's:{Research Notes of the American Astronomical Society}:{RNAAS}:g' | sed 's:{Astronomische Nachrichten}:{AN}:g' > $(TEXFILE_BASENAME).bib_tmp && mv -v $(TEXFILE_BASENAME).bib_tmp $(TEXFILE_BASENAME).bib
else
	# Nothing to do
	echo "KEEP THE ORIGINAL BIBFILE"
	echo $(MODIFY_BIBFILE_ULTRACOMPACT_REF)
endif

check_british_spelling:
ifeq ($(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING),yes)
	# Check for British spelling
	# MNRAS style guide https://academic.oup.com/mnras/pages/General_Instructions#6%20Style%20guide
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'timescale' && echo "SHOULD BE time-scale" && exit 1 || true; }
	#
	# random collection of words
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labor' && echo "SHOULD BE labour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analog' && echo "SHOULD BE analogue" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	# Other MNRAS things
	cat $(TEXFILE_BASENAME).tex | { grep --color=always --ignore-case '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\,' && echo "SHOULD BE e.g." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\.\,' && echo "SHOULD BE i.e." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case '``' && echo "SHOULD BE \`" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case "''" && echo "SHOULD BE \'" && exit 1 || true; }
else
	# Nothing to do
	echo "THIS DOES NOT LOOK LIKE A MNRAS MANUSCRIPT - NOT ENFORCING BRITISH SPELLING"
	echo $(MNRAS_MANUSCRIPT_REQUIRING_BRITISH_SPELLING)
endif

check_us_spelling:
ifeq ($(AAS_MANUSCRIPT_REQUIRING_US_SPELLING),yes)
	# Check for US spelling
	# AAS style guide https://journals.aas.org/aas-style-guide/
	# they also suggest follow The Chicago Manual of Style https://www.chicagomanualofstyle.org/home.html
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centered' && echo "SHOULD BE centred" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centred' && echo "SHOULD BE centered" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'center' && echo "SHOULD BE centre" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | grep -v '\\center' | { grep --color=always 'centre' && echo "SHOULD BE center" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulfur' && echo "SHOULD BE sulphur" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'sulphur' && echo "SHOULD BE sulfur" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labeled' && echo "SHOULD BE labelled" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'labelled' && echo "SHOULD BE labeled" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyze' && echo "SHOULD BE analyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analyse' && echo "SHOULD BE analyze" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrise' && echo "SHOULD BE parametrize" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'parametrize' && echo "SHOULD BE parametrise" && exit 1 || true; }
	# Yes, acknowledgements
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgments' && echo "SHOULD BE acknowledgements" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'acknowledgements' && echo "SHOULD BE acknowledgments" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artifact' && echo "SHOULD BE artefact" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'artefact' && echo "SHOULD BE artifact" && exit 1 || true; }
	# Yes, best-fitting seems to be OK at AAS
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fit ' && echo "SHOULD BE best-fitting" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'best-fitting ' && echo "SHOULD BE best-fit" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'disk' && echo "SHOULD BE disc" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e ' disc\,' -e ' disc\.' -e 'disc$$' -e 'disc ' && echo "SHOULD BE disk" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'halos' && echo "SHOULD BE haloes" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'haloes' && echo "SHOULD BE halos" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'hot-spot' && echo "SHOULD BE hotspot" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'nonlinear' && echo "SHOULD BE non-linear" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' onto ' && echo "SHOULD BE on to" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' on to ' && echo "SHOULD BE onto" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'time-scale' && echo "SHOULD BE timescale" && exit 1 || true; }
	#
	# random collection of words
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'color' && echo "SHOULD BE colour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'colour' && echo "SHOULD BE color" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavor' && echo "SHOULD BE flavour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'flavour' && echo "SHOULD BE flavor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humor' && echo "SHOULD BE humour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'humour' && echo "SHOULD BE humor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labor' && echo "SHOULD BE labour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v '$^{' | { grep --color=always 'labour' && echo "SHOULD BE labor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbor' && echo "SHOULD BE neighbour" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'neighbour' && echo "SHOULD BE neighbor" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyze' && echo "SHOULD BE paralyse" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'paralyse' && echo "SHOULD BE paralyze" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalog' && echo "SHOULD BE catalogue" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | sed 's:talogue::g' | { grep --color=always --ignore-case 'catalogue' && echo "SHOULD BE catalog" && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analog' && echo "SHOULD BE analogue" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'analogue' && echo "SHOULD BE analog" && exit 1 || true; }
	#
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modeling' && echo "SHOULD BE modelling" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'modelling' && echo "SHOULD BE modeling" && exit 1 || true; }
	# Other AAS things
	#cat $(TEXFILE_BASENAME).tex | { grep --color=always --ignore-case '\\%' && echo "SHOULD BE per cent" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e '~sec ' -e ' sec ' -e '\\,sec' && echo "SHOULD BE s" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\. ' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'e\.g\.\]' && echo "SHOULD BE e.g.," && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case 'i\.e\. ' && echo "SHOULD BE i.e.," && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case -e 'cf\.\,' -e ' cf ' && echo "SHOULD BE cf." && exit 1 || true; }
	#cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' etc ' && echo "SHOULD BE etc." && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always --ignore-case ' `[a-zA-Z]' && echo "SHOULD BE \`\`" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep -v "s' " | { grep --color=always --ignore-case "[a-zA-Z]' " && echo "SHOULD BE \'\'" && exit 1 || true; }
	# super AAS-specific
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'Fig\.' && echo "SHOULD BE Figure" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'Sec\.' && echo "SHOULD BE Section" && exit 1 || true; }
	#
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'errorbar' && echo "SHOULD BE error bar" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'free-fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'free fall' && echo "SHOULD BE freefall" && exit 1 || true; }
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | { grep --color=always 'free~fall' && echo "SHOULD BE freefall" && exit 1 || true; }
else
	# Nothing to do
	echo "THIS DOES NOT LOOK LIKE AN AAS MANUSCRIPT - NOT ENFORCING US SPELLING"
	echo $(AAS_MANUSCRIPT_REQUIRING_US_SPELLING)
endif

check_software_small_capitals:
ifeq ($(ANY_KNOWN_SOFTWARE_MENTIONED),yes)
	# Check that \textsc is used in the text
	echo "CHECK IF \\textsc{SoftWare} IS USED"
	cat $(TEXFILE_BASENAME).tex | cut -f1 -d"%" | grep '\\textsc'
else
	# Nothing to do
	echo "NO KNOWN SOFTWARE NAMES RECOGNIZED"
	echo $(ANY_KNOWN_SOFTWARE_MENTIONED)
endif

$(TEXFILE_BASENAME).pdf: $(TEXFILE_BASENAME).tex
ifeq ($(PDFTEX),yes)
	# pdflatex
	echo "YES PDF"
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	echo "YES BibTeX"
	echo $(BIBTEX)
	# This works with .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && { for i in *eps *png *jpg ;do if [ ! -f $$i ];then continue ;fi ; cat $(TEXFILE_BASENAME).tex | cut -f1 -d'%' | grep --quiet "$$i" && continue ; echo "WARNING: a bonus figure not included in the TeX source: $$i" ;done ; echo " " ; }  && okular $(TEXFILE_BASENAME).pdf
else
	echo "NO BibTeX"
	echo $(BIBTEX)
	# No BibTeX, .pdf/.png figures
	pdflatex $(TEXFILE_BASENAME).tex && pdflatex $(TEXFILE_BASENAME).tex && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && { for i in *eps *png *jpg ;do if [ ! -f $$i ];then continue ;fi ; cat $(TEXFILE_BASENAME).tex | cut -f1 -d'%' | grep --quiet "$$i" && continue ; echo "WARNING: a bonus figure not included in the TeX source: $$i" ;done ; echo " " ; }  && okular $(TEXFILE_BASENAME).pdf
endif

else
	# latex
	echo "NO PDF  "
	echo $(PDFTEX)
ifeq ($(BIBTEX),yes)
	echo "YES BibTeX"
	echo $(BIBTEX)
	# BibTeX and .eps figures (the right way)
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && bibtex $(TEXFILE_BASENAME) && latex $(TEXFILE_BASENAME).tex && { latex $(TEXFILE_BASENAME).tex 2>&1 | grep --color=always 'undefined on input line' && exit 1 || true; } && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && { for i in *eps *png *jpg ;do if [ ! -f $$i ];then continue ;fi ; cat $(TEXFILE_BASENAME).tex | cut -f1 -d'%' | grep --quiet "$$i" && continue ; echo "WARNING: a bonus figure not included in the TeX source: $$i" ;done ; echo " " ; } && okular $(TEXFILE_BASENAME).pdf
else
	echo "NO BibTeX"
	echo $(BIBTEX)	
	# This works with .eps figures or when \usepackage[demo]{graphicx} is activated
	latex $(TEXFILE_BASENAME).tex && latex $(TEXFILE_BASENAME).tex && dvips -o $(TEXFILE_BASENAME).ps $(TEXFILE_BASENAME).dvi && ps2pdf $(TEXFILE_BASENAME).ps && texcount -v3 -merge -incbib -dir -sub=none -utf8 -sum $(TEXFILE_BASENAME).tex && { for i in *eps *png *jpg ;do if [ ! -f $$i ];then continue ;fi ; cat $(TEXFILE_BASENAME).tex | cut -f1 -d'%' | grep --quiet "$$i" && continue ; echo "WARNING: a bonus figure not included in the TeX source: $$i" ;done ; echo " " ; } && okular $(TEXFILE_BASENAME).pdf
endif

endif
	
